Structured Training for Neural Network Transition-Based Parsing

We present structured perceptron training for neural network transition-based dependency parsing. We learn the neural network representation using a gold corpus augmented by a large number of automatically parsed sentences. Given this fixed network representation, we learn a final layer using the structured perceptron with beam-search decoding. On the Penn Treebank, our parser reaches 94.26% unlabeled and 92.41% labeled attachment accuracy, which to our knowledge is the best accuracy on Stanford Dependencies to date. We also provide in-depth ablative analysis to determine which aspects of our model provide the largest gains in accuracy.

==> tex/final.tex <==
\section{Final Results}
\newcommand\T{\rule{0pt}{4ex}}       % Top strut

\begin{table}
\scalebox{0.9}{
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l@{\hskip .3em}rcc}
\hline
\multicolumn{2}{l}{Method} & UAS & LAS \\
\hline
\hline
\multicolumn{2}{l}{\newcite{martins-etAl:2013:ACL}} & 92.20 & 89.67 \\
\multicolumn{2}{l}{\newcite{zhang-mcdonald:2014:ACL} reimpl.} & 93.22 & 91.02 \\
\multicolumn{2}{l}{\newcite{zhang-nivre:2011:ACL} reimpl.} & 93.00 & 90.95 \\

\multicolumn{2}{l}{\newcite{chen-manning:2014:EMNLP}} & 91.80 & 89.60 \T \\
\multicolumn{2}{l}{Our Softmax (B=1)} & 92.74 & 90.40 \\
\multicolumn{2}{l}{Our Perceptron (B=8)} & {\bf 93.36} & {\bf 91.30} \\
\multicolumn{2}{l}{Our Softmax+Tri-training$^\star$ (B=1)} & 93.46 & 91.49  \\
\multicolumn{2}{l}{Our Perceptron+Tri-training$^\star$ (B=8)} & {\bf 94.08} & {\bf 92.19} \\

\newcite{petrov-EtAl:2006:ACL} & F1: 90.37 & 93.61 & 91.51 \T \\
\newcite{petrov:2010:NAACL}$^\diamond$ & F1: 91.66 & 94.57 & 92.71 \\
\newcite{mcclosky-etAl:2006:NAACL}$^{\diamond\star}$ & \rule{-1cm}{0em}F1: 92.16 & 94.48 & 92.27 \\
\newcite{huang-etAl:2010:EMNLP}$^{\diamond\star}$ & F1: 92.48 & 95.05 & 93.23 \\
\hline
\end{tabular}}
\caption{\label{tab:english_final}
  Final English test set results. The top section shows the best dependency parsing accuracies
  that have been reported on Stanford dependencies; the bottom section
  shows the accuracy of constituency parsers. Baseline numbers were generated by soliciting the output
  of those system from their authors and converting it to dependencies.
  We improve over the best-reported
  Standford dependency parsers by a margin of 0.86 UAS, and over
  \newcite{chen-manning:2014:EMNLP} by 2.26 UAS. Even without tri-training, our model
  is competitive with the state-of-the-art Berkeley constituency parser.
  Re-ranking or ensemble methods are denoted by $\diamond$ and
  methods requiring parsing of unlabeled data are denoted by $\star$.}
\end{table}

Table \ref{tab:english_final} shows our final results on WSJ test set.
We compare to the best dependency parsers for which results on Stanford dependencies are available.
These results are show in the top part of the table.
The bottom part of the table shows the accuracy of the very best constituency parsers
when their output is converted to dependencies.
The reported numbers are similar to those in \newcite{kong-smith:2014} but deviate slightly since we asked
the authors for the predictions of their system on the test set and in some cases newer versions of the systems were used.

Our parser outperforms all dependency parsers and is competitive with the constituency parsers.
It should be noted that the constituency parsers (except \newcite{petrov-EtAl:2006:ACL}) use reranking,
products of experts and sometimes self-training on unlabeled data.
Despite its simplicity, our parser is within reach of these much more complex parsers.

Unfortunately we are not able to compare to several semi-supervised dependency parsers that
achieve some of the highest reported accuracies on the WSJ, in particular
\newcite{suzuki-EtAl:2009:EMNLP} and \newcite{chen-etAl:2013:EMNLP}.
These parsers use the \cite{yamada2003statistical} dependency conversion and the accuracies are
therefore not directly comparable. It should however be noted that these parsers have an
accuracy below 93.80 UAS ... finish sentence depending on what our test set accuracy is.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> tex/semi-supervised.tex <==
\section{Semi-Supervised Training}

Pre-trained embeddings are a particularly simple way of leveraging large amounts of unlabeled data,
but my no means the only one.

\newcite{petrov-EtAl:2010:EMNLP} demonstrated that a greedy transition-based parser can be
significantly improved by training it on the output of a more accurate parser.
\newcite{li-etAl:2014:ACL} improve on this idea by training only on sentences for which two different
parsers produced the same parse tree.
The intuition behind this ``tri-training'' is that the chance of two parsers agreeing is much higher when
the parse tree is correct since there is only one way to be correct while there are many possible incorrect
parses. This of course holds only as long as the parsers suffer from different biases.
In their experiments, the BerkeleyParser \cite{petrov-EtAl:2006:ACL}, latent variable constituency parser
and ZPar \cite{zhang-nivre:2011:ACL}, a transition-based parser with beam search, are used.
We follow their setup and use the same parsers to select sentences from the corpus of \newcite{1-billion-lm}.
Since unlabeled data is plentiful, we can afford to reject the majority of parses.
In our experiments the two parsers agree only 25\% of the time, but their accuracy on the
sentences that they agree on is very high ($>96\%$ UAS).


Figure \ref{fig:uptraining_results} shows that
training on the output of the BerkeleyParser and yields only modest gains,
while training on the data where the two parsers agree produces significantly better results.

% \begin{figure*}
% \centering
% \includegraphics[scale=0.6]{uptraining-UAS}\hspace*{-.5cm}\includegraphics[scale=0.6]{uptraining-LAS}
% \caption{\label{fig:uptraining_results}
% Semi-supervised training.}
% \end{figure*}
\begin{figure}
  \centering
  \includegraphics[scale=0.5]{uptraining-crop}
  \caption{Semi-supervised training with $10^7$ additional tokens. \todo{GET MISSING NUMBER!}}
  \label{fig:uptraining_results}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "train"
%%% End:

